Distributed Asynchronous Time-Varying Quadratic Programming with Asynchronous Objective Sampling

Existing works on multi-agent time-varying optimization allow agents to asynchronously communicate and/or compute, but do not allow asynchronous sampling of objectives. Sampling can be difficult to synchronize, and we therefore present a multi-agent optimization framework that allows asynchrony in sampling, communications, and computations for time-varying quadratic programs. We show that agents have bounded error when tracking the solution to the asynchronously sampled problem, which solves an open problem for quadratic programs. Simulations validate these results.

==> 4-algorithm-old.tex <==
\section{Asynchronous Update Law} \label{sec:algorithm}
% This section presents the proposed asynchronous algorithm.
\newnew{
Now we present the setup for asynchronous multi-agent optimization
of time-varying objectives with asynchronous sampling.
While one
could envision developing a  new algorithm for this setting, we show
that is not necessary. Instead, 
in Algorithm~\ref{alg:myAlg} below
we revisit and adapt the classic 
asynchronous block coordinate descent algorithm, which was shown 
in~\cite[Chapter 7]{bertsekas1989parallel} to be robust
to asynchronous communications and computations.
We show for the first time that it is robust to asynchronous
objective sampling as well. 
}

\subsection{Timescale Separation}
% Problem~\ref{prob:discrete} is indexed by the discrete time index~$\ind{}{\ell}$. We start the index~$\ell = 0$ and increment by~$1$, i.e.~$\ell \to \ell + 1$, every~$t_s$ seconds. 
% Similarly, 
Problem~\ref{prob:aggregate} is indexed by~$\ind{}{z}$.
It starts with~$z = 0$ and increments~$z$ by~$1$ at
the times at which at least one agent samples Problem~\ref{prob:discrete}.
We index agents' computations and communications over the time index~$k$ 
because these operations need not occur at the same times as their samples. 
Similar to~\cite{hauswirth2020timescale, colombino2019online}, 
we use a ``correction-only'' algorithm that does not predict changes in agents' objectives 
since it would be difficult to do so under asynchronous sampling. 
Some timescale separation is therefore required~\cite{simonetto2017decentralized}
between the changes in objectives and the agents' communications and computations.

\begin{assumption} \label{ass:timescale}
     In Problem~\ref{prob:aggregate}, for each~$\tz \in \Ts$, there are~${\kappa_z > 0}$ ticks of~$k$ when minimizing~$\g{\cdot}{\tz}$.      
     \hfill $\lozenge$ 
\end{assumption}

%\begin{remark}
   
    \gb{Eliminating Assumption~\ref{ass:timescale} would not necessarily force Algorithm~\ref{alg:myAlg} 
    fo fail     to converge, though it would make our theoretical guarantees no longer hold.}
    We use~$\eta_z \in \N$ to denote the total number of ticks of~$k$ that occur before~$\ind{}{z}$ increments to~$\ind{}{z + 1}$, i.e.,~$\eta_z = \sum^{z}_{i=0} \kappa_i$.
We set~$\kappa_{-1}=0$ and~$\eta_{-1}=0$.


\subsection{Asynchronous Block Coordinate Descent (BCD)}
We consider a block-based gradient projection algorithm with asynchronous computations and communications to track the solutions of Problem~\ref{prob:aggregate}. 
Each agent updates only a subset of the entire decision vector, and 
agents' locally updated values are then communicated to other agents over time.
Asynchrony implies that agents receive different values at different times, and thus they have different values of decision variables onboard. 
At any time~$k$, agent~$i$ has a local copy of the decision vector, denoted~$\x{i}{}{k}$.
Due to asynchrony, we allow~$\x{i}{}{k} \neq \x{j}{}{k}$ for~$i \neq j$. 
Within the vector~$\x{i}{}{k}$, agent~$i$ computes updates only to its own sub-vector of decision variables,~$\x{i}{i}{k} \in \R^{n_i}$. 
At any time~$k$, agent~$i$ has (possibly old) values for agent~$j$'s sub-vector of the decision variables, denoted by~$\x{i}{j}{k} \in \R^{n_j}$. These are updated only by agent~$j$ and then communicated by agent~$j$ to agent~$i$ and others. 

At time~$k$, if agent~$i$ computes an update to~$\x{i}{i}{k}$, then its computations use the decision vector~$\x{i}{}{k}$. 
The entries of~$\x{i}{j}{k}$ for~$j \! \neq \! i$ are obtained by communications from agent~$j$, which may be subject to delays. Therefore, agent~$i$ may (and often will) compute updates to~$\x{i}{i}{k}$ based on outdated information from other agents.

Let~$\K^i$ be the set of times at which agent~$i$ computes an update to~$\x{i}{i}{}$. 
Let~$\C^i_j$ be the set of times at which agent~$i$ receives a transmission of~$\x{j}{j}{}$ from agent~$j$; due to communication delays, these transmissions can be received long after they are sent, and they can be received at different times by different agents. The sets~$\K^i$ and~$\C^i_j$ are only defined to simplify discussion and analysis, and
agents do not need to know them. 
We define~$\tau^i_j(k)$ to be the time at which agent~$j$ originally computed the value of~$\x{i}{j}{k}$ that agent~$i$ has onboard at time~$k$. 
At time~$k$, agent~$i$ stores the vector
\begin{equation}
    \x{i}{}{k} = \left( \x{1}{1}{\tau^i_1(k)}^T,\dots,\x{i}{i}{k}^T,\dots, \x{N}{N}{\tau^i_N(k)}^T \right)^T. \label{eq:1000} 
\end{equation}
We will also analyze the true state of the network, namely 
\begin{equation}
    \x{}{}{k} = \left( \x{1}{1}{k}^T,\x{2}{2}{k}^T,\dots,\x{N}{N}{k}^T \right)^T . \label{eq:1001}
\end{equation} 
We assume that computation and communication delays are bounded, which has been called \emph{partial asynchrony}~\cite{bertsekas1989parallel}. 

\begin{assumption} \label{ass:partialAsynch}
There exists~$B \in \N$ such that
    \begin{enumerate}
    \item For all $i \in [N]$ and all $k \geq 0$, at least one element
    of the set $\left\{ k,k+1,\dots,k+B-1\right\} $ belongs to $\K^{i}$
    \item The bound
    %\begin{equation}
    $\max\left\{ 0,k-B+1\right\} \leq\tau_{j}^{i}\left(k\right)\leq k$
    %\end{equation}
     holds for all $i \in [N]$, $j \in [N]$, and~$k \geq 0$. \hfill $\lozenge$
    \end{enumerate} 
\end{assumption}

\gb{Assumption~\ref{ass:partialAsynch} only needs
to hold for some~$B \in \N$, and that~$B$ does not need to be small. 
It cannot be removed since unbounded delays
can cause divergence~\cite[Section 6.3]{bertsekas1989parallel}. 
}
%We will use it to prove that for each~$\tz \in \Ts$ our algorithm makes progress toward some element of~$\X^*(\tz)$ across intervals of~$B$ time steps (or multiples of~$B$ time steps). 
% \gb{We could reference back to our timescale assumption here and say the partial asynchrony assumption here requires the specific form of the iterates, i.e.,~$\kappa_z = \chi_z + r_zB$. I can also see how talking about that assumption again could raise concerns in the reviewer if we defend it too much. Let me know what you think.}
% For simplicity, for each~$\tz \in \T$ and for some~$v_z \in \N$, we consider~$\kappa_z = v_z B$. Furthermore, we adopt the convention that~$\kappa_{-1}=0$ and~$\eta_{-1}=0$.

%We require a  algorithm that is robust to asynchrony and can be distributed.  
%Therefore, 
%To do so, we propose the projected-gradient update law
We propose to use the projected gradient update law 
\begin{align}
\x{i}{i}{k+1}= & \begin{cases}
\Omega_i \big( \x{i}{}{k} \big) & k\in \K^{i}\\
\x{i}{i}{k} & k\notin \K^{i}
\end{cases}\label{eq:update}  \\
\x{i}{j}{k+1}= & \begin{cases}
\x{j}{j}{\tau_{j}^{i}(k)} & k\in \C_{j}^{i}\\
\x{i}{j}{k} & k\notin \C_{j}^{i}
\end{cases},
\end{align}
where
\begin{equation}
    \Omega_i \big(\x{i}{}{k}\big) 
    = \Pi_{\X_{i}} \Big[\x{i}{i}{k} 
     - \gamma_z \big( Q^{[i]} (\theta_i ( \tz ) ) \x{i}{}{k} + r^{[i]}(\theta_i ( \tz )) \big)\Big]
\end{equation}
and~$\gammaz > 0$ is the step size. 
Agents' communications
are \emph{not} all-to-all. Instead, two agents communicate only if
one’s updates rely upon the other’s sub-vector of decision
variables. 
Algorithm~\ref{alg:myAlg} provides pseudocode for agents' updates. 


\begin{algorithm}[t!]
    \caption{Asynchronous Projected BCD}
    \label{alg:myAlg}
	\SetAlgoLined
	\KwIn{$\x{i}{j}{0}$ for all~$i,j \in [N]$}
	\For{$\tz \in \Ts$}
	{
		\For{$k=\eta_{z-1}+1:\eta_{z}$}
		{
			\For{i=1:N}
			{
			    \For{j=1:N}
			    {
    				\If{$k \in \C^{i}_j$}{    			
                        ~\phantom{} $\x{i}{j}{k+1} = \x{j}{j}{\tau^i_j(k)}$ 
    				}
    				\Else{
    				    ~\phantom{} $\x{i}{j}{k+1} = \x{i}{j}{k}$
    				}
    			}
				\If{k $\in \K^{i}$ }{
					~$\x{i}{i}{k+1} = \Omega_i \left( \x{i}{}{k} \right) $
				}
				\Else{
				~$\x{i}{i}{k+1} = \x{i}{i}{k}$ 
				}
			}			
		}	
	}
\end{algorithm}



==> 8-biographies.tex <==
\vspace{-4\baselineskip}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio,draft=false]{bioPics/BEHRENDT_GABRIEL.pdf}}] {Gabriel Behrendt} received the B.S. degree in Mechanical Engineering from the University of Iowa in 2020, and the M.S. degree in Aerospace Engineering from the University of Florida in 2022. He is currently pursuing a Ph.D. in Electrical and Computer Engineering at Georgia Tech. His research interests include time-varying optimization and applications to aerospace systems with an emphasis on asynchronous multi-agent systems and distributed optimization.
\end{IEEEbiography}

\vspace{-4\baselineskip}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio,draft=false]{bioPics/BELL_ZACHARY_I-min-min.pdf}}] {Zachary I. Bell} received his Ph.D. from the University of Florida in 2019 and is a researcher for the Air Force Research Lab. His research focuses on cooperative guidance and control, computer vision, adaptive control, and reinforcement learning.
\end{IEEEbiography}

\vspace{-3.5\baselineskip}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio,draft=false]{bioPics/hale.pdf}}] {Matthew Hale} is an Associate Professor of Electrical and Computer Engineering at Georgia Tech. He received his PhD in Electrical and Computer Engineering from Georgia Tech in 2017. His research interests include multi-agent systems, mobile robotics, and privacy in control. He has received the
the NSF CAREER Award, ONR YIP, and AFOSR YIP.
\end{IEEEbiography}

==> Lemmas/0-upperConvexityBound.tex <==
\begin{lemma} \label{lem:upperConvexity}
    For each~$ \tz \in \Ts$ and all~$x \in \X$, the function~$\mathcal{S} \ni h: \R^n \times \R_+ \rightarrow \R$ 
    defined as~$\h{x}{\tz} = \frac{1}{2}\|x\|^2 + M_{g, z}$ satisfies~$\h{x}{\tz} \geq \g{x}{\tz}$. 
    % \begin{align}
    %     \h{x}{\tz} \geq \g{x}{\tz}
    % \end{align}
\end{lemma}
\noindent \emph{Proof.} From Assumption~\ref{ass:setConstraint} and the continuity of~$\g{\cdot}{\tz}$ for all~$\tz \in \Ts$ there exists~$M_{g,z} > 0$ such that~$\g{x}{\tz} \leq M_{g, z}$ for all~$x \in \X$.
Then~$h(x; t_z) \geq g(x; t_z)$ for all~$x \in \X$. 
%Defining~$h(x; t_z) \coloneqq \frac{1}{2}\|x\|^2 + M_{g, z}$ yields the result.
% \begin{equation}
%     h(x; t_z) = \frac{1}{2}\|x\|^2 + M_{g, z} 
% \end{equation}
% and~$h(x; t_z) \geq g(x; t_z)$ for all~$x \in \X$. 
\hfill $\blacksquare$


\begin{lemma} \label{lem:balls}
    Let~$m$ denote the Lebesgue measure. 
    Assume~$D \subset \R^d$ is convex, compact, and has nonempty interior and let~$r_\X > 0$ denote its inradius. 
    Then there exists~$\nu_\X \in (0,1)$ such that~$m \big( \B(x,r) \cap D \big) \geq \nu_\X m \big( \B(x,r) \big)$,
    % \begin{align}
    %     m \big( \B(x,r) \cap D \big) \geq \lambda_\X m \big( \B(x,r) \big),
    % \end{align}
    for any~$x \in \X$ and~$r \leq r_\X$.
\end{lemma}
\noindent \emph{Proof.}
See~\cite[Lemma A.1]{nozari2016differentially}.
\hfill $\blacksquare$





==> Lemmas/1-jorgeBound.tex <==
\subsection{Proof of Lemma~\ref{lem:argmin}} \label{lem:jorge}
    Let~$a = \argmin_{x \in \X} \f{x}{\tz}$ and $b = \argmin_{x \in \X} \h{x}{\tz}$ where~$a \neq b$. Let~$m_a = \f{a}{\tz}$,~$m_b=\h{b}{\tz}$,~$m = m_a - m_b$,~$u_a = \nabla_x \f{a}{\tz}$, and~$u_b = \nabla_x \h{b}{\tz}$. Without loss of generality, assume~$m \geq 0$. 
    Then~\cite[Proposition A.2]{nozari2016differentially} gives
    %For all~$a,b,x \in \X$, define,
    %\begin{align}
    %    \fl{x}{\tz} = \frac{\varphi}{2} \| x-a \|^2 + u_a^T(x-a) + m_a \label{eq:1009}\\
    %    \hu{x}{\tz} = \frac{\psi}{2} \| x-b \|^2 + u_b^T(x-b) + m_b \label{eq:1010}.
    %\end{align}
    %Differentiating~\eqref{eq:1009} and~\eqref{eq:1010} twice with respect to~$x$ we get
    %%\begin{equation}
    %    $\nabla_x^2 \fl{x}{\tz}  = \varphi I_n$ and
    %    $\nabla_x^2 \hu{x}{\tz} = \psi I_n$.
    %%\end{equation}
    %Since~$f,h \in \mathcal{S}$, 
    %\begin{equation}
    %    \nabla_x^2 \f{x}{\tz} \succeq \varphi I_n \quad \textnormal{ and } \quad
    %    \nabla_x^2 \h{x}{\tz} \preceq \psi I_n \label{eq:1012} .
    %\end{equation}
    %Using the same steps as in~\cite[Proposition~A.2]{nozari2016differentially}, 
    %we see that
  %  Since~$f,h \in C^2(\X) \subset L_2(\X)$ we integrate~\eqref{eq:1011} and~\eqref{eq:1012} twice to obtain
  %  \begin{equation}
  %      \fl{x}{\tz} \leq \f{x}{\tz}, \quad
  %      \hu{x}{\tz} \geq \h{x}{\tz},
  %  \end{equation}
  %  for all~$x \in \X$. It follows that, for all~$x \in \X$,
  %  \begin{align}
  %      | \f{x}{\tz} - \h{x}{\tz} | &\geq [ \fl{x}{\tz} - \hu{x}{\tz} ]^+ \\
  %      &\geq [ \fl{x}{\tz} - \hu{x}{\tz} - m ]^+ \label{eq:1015}
  %  \end{align}
  %  where~$[z]^+ = \max \{ z,0 \}$ for~$z \in \R$. 
  %    
  %  \begin{align}
  %      \fl{x}{\tz} - \hu{x}{\tz} - m = - \frac{\psi - \varphi}{2} \Big( \|x-c \|^2  -   r^2 \Big),
  %  \end{align}
  % over~$\B(c, r)$, where
  %  \begin{align}
  %      c &= \frac{\psi b - \varphi a + u_a - u_b}{\psi - \varphi}, \\
  %      r^2 &=   \frac{ \varphi \psi \| a-b \|^2}{(\psi - \varphi)^2}
  %       + \frac{ \| u_a - u_b \|^2}{(\psi - \varphi)^2}
  %       + \frac{2 ( b - a )^T ( \psi u_a - \varphi u_b)}{(\psi - \varphi)^2}.  \label{eq:1013}
  %  \end{align}
  %  Therefore, 
  %the region where~$\fl{\cdot}{\tz} - \hu{\cdot}{\tz} - m \geq 0$ is~$\B(c,r)$, where
  %  \begin{align}
  %      c &= \frac{\psi b - \varphi a + u_a - u_b}{\psi - \varphi}, \\
  %      r^2 &=   \frac{ \varphi \psi \| a-b \|^2}{(\psi - \varphi)^2}
  %       + \frac{ \| u_a - u_b \|^2}{(\psi - \varphi)^2}
  %       + \frac{2 ( b - a )^T ( \psi u_a - \varphi u_b)}{(\psi - \varphi)^2},  \label{eq:1013}
  %  \end{align}
  %  and~$\B(c,r)$ is an open ball centered at~$c$ with radius~$r>0$.
%    Next, we find a subset of~$\B(c,r)$ where we can find a positive lower bound on~$f_l - h_u$ that depends on~$\| a-b \|$.
   % We note as well that 
%    \begin{align}
%        r^2 - \| b - c \|^2 &=  r^2
%         - \bigg\| b - \frac{\psi b - \varphi a + u_a - u_b}{\psi - \varphi} \bigg\|^2
%    \end{align}
%    After some expansion, rearranging, and plugging in the definition of~$r^2$ in~\eqref{eq:1013} we find
    %\begin{align}
    %    r^2 - \| b - c \|^2 &= \frac{  \varphi  }{ \psi - \varphi } \| a - b \|^2 
    %    + \frac{ 2 }{ \psi - \varphi } u_a^T ( b-a ). \label{eq:1014} 
    %\end{align}
    %
    % Expanding this expression yields
    % \begin{align}
    %     r^2 - \| b - c \|^2 &=  r^2
    %      - \bigg(  b - \frac{\psi b - \varphi a + u_a - u_b}{\psi - \varphi} \bigg)^T 
    %      \bigg(  b - \frac{\psi b - \varphi a + u_a - u_b}{\psi - \varphi} \bigg) \\
    %      &= r^2
    %      - \bigg( b^T b - 2 b^T \bigg( \frac{\psi b - \varphi a + u_a - u_b}{\psi - \varphi} \bigg) + \bigg( \frac{\psi b - \varphi a + u_a - u_b}{\psi - \varphi} \bigg)^T \bigg( \frac{\psi b - \varphi a + u_a - u_b}{\psi - \varphi}  \bigg)  \bigg)  \\
    %      &= r^2
    %      - \bigg( b^T b -  \bigg( \frac{2 \psi b^T b - 2 \varphi b^T a + 2 b^T u_a - 2 b^T u_b}{\psi - \varphi} \bigg)  \\
    %      &+ \bigg( \frac{\psi^2 b^T b - 2 \varphi \psi b^T a + 2 \psi b^T u_a - 2 \psi b^T u_b + \varphi^2 a^T a - 2 \varphi a^T u_a + 2 \varphi a^T u_b + u_a^T u_a - 2 u_a^T u_b + u_b^T u_b}{( \psi - \varphi )^2}  \bigg) 
    % \end{align}
    % % Still expanding...
    % %     \begin{align}
    % %     r^2 - \| b - c \|^2 &=  r^2
    % %      - \bigg(  b - \frac{\psi b - \varphi a + u_a - u_b}{\psi - \varphi} \bigg)^T 
    % %      \bigg(  b - \frac{\psi b - \varphi a + u_a - u_b}{\psi - \varphi} \bigg) \\
    % %      &= r^2
    % %      - \bigg( b^T b - 2 b^T \bigg( \frac{\psi b - \varphi a + u_a - u_b}{\psi - \varphi} \bigg) + \bigg( \frac{\psi b - \varphi a + u_a - u_b}{\psi - \varphi} \bigg)^T \bigg( \frac{\psi b - \varphi a + u_a - u_b}{\psi - \varphi}  \bigg)  \bigg)  \\
    % %      &= r^2
    % %      - \bigg( b^T b -  \bigg( \frac{2 \psi b^T b - 2 \varphi b^T a + 2 b^T u_a - 2 b^T u_b}{\psi - \varphi} \bigg)  \\
    % %      &+ \bigg( \frac{\psi^2 b^T b - 2 \varphi \psi b^T a + 2 \psi b^T u_a - 2 \psi b^T u_b + \varphi^2 a^T a - 2 \varphi a^T u_a + 2 \varphi a^T u_b + u_a^T u_a - 2 u_a^T u_b + u_b^T u_b}{( \psi - \varphi )^2}  \bigg) 
    % % \end{align}
    % Multiplying the second term by~$\frac{\psi - \varphi}{\psi - \varphi}$ and expanding gives us
    % \begin{align}
    %      &= r^2
    %      - \bigg( b^T b 
    %      -  \bigg( \frac{(2 \psi b^T b - 2 \varphi b^T a + 2 b^T u_a - 2 b^T u_b) (\psi - \varphi)}{(\psi - \varphi)(\psi - \varphi)} \bigg)  \\
    %      &+ \bigg( \frac{\psi^2 b^T b - 2 \varphi \psi b^T a + 2 \psi b^T u_a - 2 \psi b^T u_b + \varphi^2 a^T a - 2 \varphi a^T u_a + 2 \varphi a^T u_b + u_a^T u_a - 2 u_a^T u_b + u_b^T u_b}{( \psi - \varphi )^2}  \bigg) \\
    %      &= r^2
    %      - \bigg( b^T b 
    %      +  \bigg( \frac{ - 2 \psi^2 b^T b + 2 \varphi \psi b^T a - 2 \psi b^T u_a + 2 \psi b^T u_b + 2 \varphi \psi b^T b - 2 \varphi^2 b^T a + 2 \varphi b^T u_a - 2 \varphi b^T u_b }{(\psi - \varphi)^2} \bigg)  \\
    %      &+ \bigg( \frac{\psi^2 b^T b - 2 \varphi \psi b^T a + 2 \psi b^T u_a - 2 \psi b^T u_b + \varphi^2 a^T a - 2 \varphi a^T u_a + 2 \varphi a^T u_b + u_a^T u_a - 2 u_a^T u_b + u_b^T u_b}{( \psi - \varphi )^2}  \bigg) \\
    % \end{align}
    % Canceling out some terms gives us
    % \begin{align}
    %      &= r^2
    %      - \bigg( b^T b 
    %      +  \bigg( \frac{ - \psi^2 b^T b   + 2 \varphi \psi b^T b - 2 \varphi^2 b^T a + 2 \varphi b^T u_a - 2 \varphi b^T u_b }{(\psi - \varphi)^2} \bigg)  \\
    %      &+ \bigg( \frac{ \varphi^2 a^T a - 2 \varphi a^T u_a + 2 \varphi a^T u_b + u_a^T u_a - 2 u_a^T u_b + u_b^T u_b}{( \psi - \varphi )^2}  \bigg)
    % \end{align}
    % Multiplying the~$b^T b$ term by~$\frac{(\psi - \varphi)^2}{(\psi - \varphi)^2}$ and expanding gives us
    % \begin{align}
    %      &= r^2
    %      - \bigg(  \frac{ \psi^2 b^T b -2 \varphi \psi b^T b + \varphi^2 b^T b}{(\psi - \varphi)^2}
    %      +   \frac{ - \psi^2 b^T b    + 2 \varphi \psi b^T b - 2 \varphi^2 b^T a + 2 \varphi b^T u_a - 2 \varphi b^T u_b }{(\psi - \varphi)^2}   \\
    %      &+ \frac{ \varphi^2 a^T a - 2 \varphi a^T u_a + 2 \varphi a^T u_b + u_a^T u_a - 2 u_a^T u_b + u_b^T u_b}{( \psi - \varphi )^2} \bigg)
    % \end{align}
    % Canceling out some terms and simplifying gives us
    % \begin{align}
    %      &= r^2
    %      -  \bigg( \frac{ \varphi^2 b^T b - 2 \varphi^2 b^T a + 2 \varphi b^T u_a - 2 \varphi b^T u_b + \varphi^2 a^T a - 2 \varphi a^T u_a + 2 \varphi a^T u_b + u_a^T u_a - 2 u_a^T u_b + u_b^T u_b}{(\psi - \varphi)^2} \bigg)
    % \end{align}
    % Now plugging in the definition of~$r^2$ from Equation~\eqref{eq:1013}
    % \begin{align}
    %      &=  \frac{ \varphi \psi \| a-b \|^2}{(\psi - \varphi)^2}
    %      + \frac{ \| u_a - u_b \|^2}{(\psi - \varphi)^2}
    %      + \frac{2 ( b - a )^T ( \psi u_a - \varphi u_b)}{(\psi - \varphi)^2} \\
    %      &-  \frac{ \varphi^2 b^T b - 2 \varphi^2 b^T a + 2 \varphi b^T u_a - 2 \varphi b^T u_b + \varphi^2 a^T a - 2 \varphi a^T u_a + 2 \varphi a^T u_b + u_a^T u_a - 2 u_a^T u_b + u_b^T u_b}{(\psi - \varphi)^2} 
    % \end{align}
    % Expanding this expression yields
    % \begin{align}
    %      &=  \frac{ \varphi \psi a^T a - 2 \varphi \psi a^T b + \varphi \psi b^T b}{(\psi - \varphi)^2}
    %      + \frac{ u_a^T u_a - 2 u_a^T u_b + u_b^T u_b }{(\psi - \varphi)^2}
    %      + \frac{ 2 \psi b^T u_a - 2 \varphi b^T u_b - 2 \psi a^T u_a + 2 \varphi a^T u_b }{(\psi - \varphi)^2} \\
    %      &-   \frac{ \varphi^2 b^T b - 2 \varphi^2 b^T a + 2 \varphi b^T u_a - 2 \varphi b^T u_b + \varphi^2 a^T a - 2 \varphi a^T u_a + 2 \varphi a^T u_b + u_a^T u_a - 2 u_a^T u_b + u_b^T u_b}{(\psi - \varphi)^2} 
    % \end{align}
    % Canceling out some terms gives us
    % \begin{align}
    %      &=  \frac{ \varphi \psi a^T a - \varphi^2 a^T a + 2 \varphi a^T u_a - 2 \psi a^T u_a  + \varphi \psi b^T b - \varphi^2 b^T b - 2 \varphi \psi a^T b + 2 \varphi^2 a^T b  + 2 \psi b^T u_a - 2 \varphi b^T u_a   }{(\psi - \varphi)^2}  
    % \end{align}
    % Combining like terms and simplifying yields
    % \begin{align}
    %      &=  \frac{ (\varphi \psi - \varphi^2 ) a^T a 
    %      - 2 ( \varphi \psi - \varphi^2 )  a^T b 
    %      + (\varphi \psi - \varphi^2 ) b^T b 
    %      + ( 2 \varphi - 2 \psi ) a^T u_a   
    %       + ( 2 \psi - 2 \varphi ) b^T u_a   }{(\psi - \varphi)^2}  \\
    %     &=  \frac{ ( \psi - \varphi ) \varphi  }{(\psi - \varphi)^2} \| a - b \|^2 
    %     + \frac{ 2 ( \psi - \varphi ) }{(\psi - \varphi)^2} u_a^T ( b-a ) \\
    %     &=  \frac{  \varphi  }{ \psi - \varphi } \| a - b \|^2 
    %     + \frac{ 2 }{ \psi - \varphi } u_a^T ( b-a )
    % \end{align}
%    If~$b \in \B(c,r)$, then~$r^2 - \| b - c \|^2 \geq 0$. 
%     We have
%     \begin{align}
%         r^2 - \| b - c \|^2 &= \frac{  \varphi  }{ \psi - \varphi } \| a - b \|^2 
%         + \frac{ 2 }{ \psi - \varphi } u_a^T ( b-a ). \label{eq:1014} 
%     \end{align}
    %Due to the strong convexity of~$f,h$ we have~$u_a^T (b-a) \geq 0$. This inequality and the fact that~$0< \varphi < \psi$ imply
    %    $r^2 - \| b - c \|^2 > 0$.
    %Therefore~$b \in \B(c,r)$. Let~$\underline{r} \coloneqq r - \| b - c \| > 0$ be the radius of the largest ball centered at~$b$ and contained in~$\B(c,r)$. %From~\eqref{eq:1014} we have the bound
    %Then we have the bound  $r^2 - \| b - c \|^2 \geq \frac{  \varphi  }{ \psi - \varphi } \| a - b \|^2$, 
    %which implies the inequality
    %%\begin{align}
    %    $\big( r - \| b - c \| \big) \big( r + \| b - c \| \big) \geq \frac{  \varphi  }{ \psi - \varphi } \| a - b \|^2$ . 
    %%\end{align}
    %Dividing both sides by~$\big( r + \| b - c \| \big)$ yields
    %\begin{align}
    %    r - \| b - c \|  &\geq \frac{\frac{ \varphi }{ \psi - \varphi } \| a - b \|^2 }{  r + \| b - c \|  } . 
    %\end{align}
    %Continuing to follow~\cite[Proposition~A.2]{nozari2016differentially}, we reach
    %
    %Due to the definition of~$\underline{r}$ and the fact~$\| b - c \| < r$ we can rewrite this as follows
    %\begin{align}
    %    \underline{r}  &\geq \frac{\frac{ \varphi }{ \psi - \varphi } \| a - b \|^2 }{  2r  } . 
    %\end{align}
    %%    Using the definition of~$r^2$ in~\eqref{eq:1013} we can write
    %\begin{align}
    %    \underline{r}  &\geq \frac{\frac{ \varphi }{ \psi - \varphi } \| a - b \|^2 }{  2 \sqrt{\frac{\varphi \psi \|a-b\|%^2 + 2 (\psi u_a - \varphi u_b)^T (b-a) + \| u_a -u_b \|^2 }{(\psi - \varphi)^2} }  } . 
    %\end{align}
    %Simplifying the denominator, using the Cauchy-Schwarz and triangle inequality, and the fact~$\| u_a \|, \| u_b \| \leq \bar{u}$ since~$f,h \in \mathcal{S}$ we find
     %\begin{align}
     %   \underline{r}  &\geq \mu_{\varphi,\psi} (\| a - b \|) , \label{eq:1017}
     %\end{align}
    %where
    %\begin{align}
    %    \mu_{\varphi,\psi} (r) &\coloneqq \frac{ \varphi r^2 }{  2 \sqrt{ \varphi \psi r^2 + 2 ( \psi  + \varphi ) \bar{u} r + 4 \bar{u}^2  }  } . \label{eq:1018} 
    %\end{align}
    %Next, note that for all~$x \in \B \big( c, \frac{r+\|c-b\|}{2} \big)$
    %\begin{multline}
    %    \fl{x}{\tz} - \hu{x}{\tz} - m \geq \\
    %    - \frac{\psi -\varphi}{2} \Big( \frac{r^2 + \|c-b\|^2 +2r \|c-b\| }{4} - r^2 \Big).
    %\end{multline}
    %Using~$2 r \| c-b \| \leq r^2 + \|c-b\|^2 $, we combine terms to find 
    %\begin{align}
    %    \fl{x}{\tz} - \hu{x}{\tz} - m 
    %    \geq \frac{  \varphi  }{ 4 } \| a - b \|^2 +  \frac{ 1 }{ 2 } u_a^T ( b-a )
    %    %&\geq - \frac{\psi -\varphi}{2} \Big( \frac{ r^2 + \|c-b\|^2 }{2} - r^2 \Big) \\
    %    %\geq - \frac{\psi -\varphi}{4} \Big( \|c-b\|^2 - r^2 \Big).
    %\end{align}
%    Substituting~$\|c-b\|^2 - r^2$ from~\eqref{eq:1014} and simplifying yields
    %\begin{multline}
    %    %\fl{x}{\tz} - \hu{x}{\tz} - m \geq 
    %    %- \frac{\psi -\varphi}{4} \Big(  - \frac{  \varphi  }{ \psi - \varphi } \| a - b \|^2 \\
    %    %- \frac{ 2 }{ \psi - \varphi } u_a^T ( b-a )  \Big) \\
    %    \geq  
    %    \frac{  \varphi  }{ 4 } \| a - b \|^2 
    %    +  \frac{ 1 }{ 2 } u_a^T ( b-a ).
    %\end{multline}
    %Due to convexity we have~$u_a^T ( b-a ) \geq 0$, so therefore
    %\begin{align}
    %     \fl{x}{\tz} - \hu{x}{\tz} - m &\geq  \frac{  \varphi  }{ 4 } \| a - b \|^2, \label{eq:1016}
    %\end{align}
    %for all~$x \in \B(b, \frac{\underline{r}}{2}) \subset \B \big(c, \frac{r + \|c - b\|}{2} \big) $. 
    %Then, from the definition of the~{$L^2$-norm} we have
    %\begin{align}
    %    \| \f{\cdot}{\tz} - \h{\cdot}{\tz} \|_{L^2}^2 = \int_\X | \f{x}{\tz} - \h{x}{\tz} |^2 dx .
    %\end{align}
%    Applying~\eqref{eq:1015} yields
    %Define~$\chi \coloneqq \f{\cdot}{\tz} - \h{\cdot}{\tz}$. Since~$\fl{x}{\tz} \leq \f{\cdot}{\tz}$ and~$\hu{x}{\tz} \geq \h{x}{\tz}$ we have
    %\begin{equation}
    %    \| \chi \|_{L^2}^2 
    %    \geq \int_\X \Big( \big[ \fl{x}{\tz} - \hu{x}{\tz} - m \big]^+ \Big)^2 dx .
    %\end{equation}
    %where~$[z]^+ = \max\{z,0\}$ for any~$z\in \R$. From above we have~$\fl{x}{\tz} - \hu{x}{\tz} - m > 0$, so then we have~$\big[ \fl{x}{\tz} - \hu{x}{\tz} - m \big]^+ = \fl{x}{\tz} - \hu{x}{\tz} - m $. Then using the fact~$ \B(b, \frac{\underline{r}}{2}) \cap \X \subset \X$ we find 
    %\begin{equation}
    %    \| \chi \|_{L^2}^2 
    %    \geq \int_{\B(b, \frac{\underline{r}}{2}) \cap \X} ( \fl{x}{\tz} - \hu{x}{\tz} - m  )^2 dx .
    %\end{equation}
    %Applying~\eqref{eq:1016} yields
    %\begin{equation}
    %    \| \chi \|_{L^2}^2 \geq 
    %    % \int_{\B(b, \frac{\underline{r}}{2}) \cap \X} 
    %    % \Big( \frac{  \varphi  }{ 4 } \| a - b \|^2  \Big)^2 dx \\
    %      \frac{  \varphi^2  }{ 16 } \| a - b \|^4 
    %    \int_{\B(b, \frac{\underline{r}}{2}) \cap \X} 1 \ dx .
    %\end{equation}
    %Integrating this expression yields
    %\begin{align}
    %    \| \chi \|_{L^2}^2  &\geq 
    %    \frac{  \varphi^2  }{ 16 } \| a - b \|^4 m \bigg( \B \left( b, \frac{\underline{r}}{2} \right) \cap \X \bigg),
    %\end{align}
    %where~$m(\cdot)$ denotes the Lebesgue measure. Applying the above we find
    %\begin{equation}
    %    \| \chi \|_{L^2}^2  \geq 
    %    \frac{  \varphi^2  }{ 16 } \| a - b \|^4 
    %    m \bigg( \B \left( b, \frac{ \mu_{\varphi,\psi} (\|a-b\|)}{2} \right) \cap \X \bigg) .
    %\end{equation}
    %Lastly, we will focus on explicitly bounding the RHS of this expression. From~\eqref{eq:1018} we have
    %\begin{align}
    %    \mu_{\varphi,\psi} (\| a - b \|) &= \frac{ \varphi \| a - b \|^2 }{  2 \sqrt{ \varphi \psi \| a - b \|^2 + 2 ( \psi  + \varphi ) \bar{u} \| a - b \| + 4 \bar{u}^2  }  } . 
    %\end{align}
    %We have~$\mu_{\varphi,\psi} (\| a - b \|) \leq \| a - b \| \leq d_\X$ for all~$a,b \in \X$. Therefore~$\frac{r_\X}{d_\X} \frac{ \mu_{\varphi,\psi} (\| a - b \|) }{2} \leq \min \Big\{ r_\X, \frac{ \mu_{\varphi,\psi} (\| a - b \|) }{2} \Big\}$. Therefore,
    %\begin{equation}
    %    \| \chi \|_{L^2}^2  \geq 
    %    \frac{  \varphi^2  }{ 16 } \| a - b \|^4 
    %    m \bigg( \B \left( b, \frac{ r_\X \mu_{\varphi,\psi} (\| a - b \|)}{2 d_\X} \right) \cap \X \bigg) .
    %\end{equation}
    %By Assumption~\ref{ass:setConstraint},~$\X$ is convex, compact, and has a nonempty interior. Thus, applying Lemma~\ref{lem:balls} yields,
    %\begin{equation}
    %    \| \chi \|_{L^2}^2  \geq 
    %    \frac{  \varphi^2  }{ 16 } \| a - b \|^4 \nu_\X 
    %    m \bigg( \B \left( b, \frac{ r_\X \mu_{\varphi,\psi} (\| a - b \|)}{2 d_\X} \right) \bigg) ,
    %\end{equation}
    %for some~$\nu_\X \in (0,1)$.
    %Applying the equation for the Lebesgue measure of a ball, i.e.~$m \left( \B (c,r) \right) = \frac{\pi^{n/2}}{ %\Gamma \left( \frac{n}{2} + 1 \right)} r^n$~\cite{NIST:DLMF}, and the fact~$\Gamma \left( \frac{n}{2} + 1 \right) = \frac{n}{2} \Gamma \left( \frac{n}{2} \right)$ where~$\Gamma(\cdot)$ is the Gamma function yields
    %\begin{equation}
    %    \| \chi \|_{L^2}^2  \geq 
    %    \frac{  \varphi^2  }{ 16 } \| a - b \|^4 \nu_\X \frac{2 \pi^{n/2}}{n \Gamma \left( \frac{n}{2} \right)} 
    %    \bigg( \frac{ r_\X \mu_{\varphi,\psi} (\| a - b \|)}{2 d_\X} \bigg)^n .
    %\end{equation}
    %\gb{Here is where we depart from Erfan's paper (Prop. A.2). Everything up to this point is identical.}
    %Rearranging this expression is equivalent to the following, 
    %\begin{equation}
    %    \| \chi \|_{L^2}^2  \geq 
    %    \frac{ \varphi^2 \pi^{n/2} }{ n 2^{n+3} \Gamma \left( \frac{n}{2} \right)  } \nu_\X \bigg( \frac{r_\X}{d_\X} \bigg)^n  \| a - b \|^4  
    %     \mu_{\varphi,\psi} (\| a - b \|)^n.
    %\end{equation}
    %
    \begin{equation}
        \| \chi \|_{L^2}^2  \geq 
        \frac{ \varphi^2 \pi^{n/2} }{ n 2^{n+3} \Gamma \left( \frac{n}{2} \right)  } \nu_\X \bigg( \frac{r_\X}{d_\X} \bigg)^n  \| a - b \|^4 
         \left( \frac{ \varphi \| a - b \|^2 }{  2 \sqrt{ \varphi \psi \| a - b \|^2 + 2 ( \psi  + \varphi ) \bar{u} \| a - b \| + 4 \bar{u}^2  }  } \right)^n,
    \end{equation}
    where~$\chi \coloneqq \f{\cdot}{\tz} - \h{\cdot}{\tz}$. 
    % \red{Shouldn't~$\chi$ be the~$L^2$ norm of that?}
    We now extend that result to 
    derive an explicit bound on~$\| \f{\cdot}{\tz} - \h{\cdot}{\tz} \|_{L^2}^2$. First, we define
    %\begin{align}
        $K_1 = \frac{ \varphi^2 \pi^{n/2} }{ n 2^{n+3} \Gamma ( \frac{n}{2} )  } \nu_\X \big( \frac{r_\X}{d_\X} \big)^n$.
    %\end{align}
    With~$\varphi < \psi$, we then have
    %Then we can write this out as
    %\begin{multline}
    %    \| \chi \|_{L^2}^2  \geq 
    %    K_1    \| a - b \|^4  \\
    %    \bigg( \frac{ \varphi \| a - b \|^2 }{  2 \sqrt{ \varphi \psi \| a - b \|^2 + 2 ( \psi  + \varphi ) \bar{u} \| a - b \| + 4 \bar{u}^2  }  } \bigg)^n.
    %\end{multline}
    %From the fact~$\varphi < \psi$ we have
    \begin{equation}
        \| \chi \|_{L^2}^2  \geq 
        K_1    \| a - b \|^4  
        \bigg( \frac{ \varphi \| a - b \|^2 }{  2 \big(\psi \| a - b \| + 2 \bar{u}\big)  } \bigg)^n, 
    \end{equation}
    where we have also used
    $\psi^2 \| a - b \|^2 + 4 \psi  \bar{u} \| a - b \| + 4 \bar{u}^2 = \left( \psi \| a - b \| + 2 \bar{u} \right)^2$. 
    %\begin{align}
    %    \| \chi \|_{L^2}^2  &\geq 
    %    K_1    \| a - b \|^4  
    %    \bigg( \frac{ \varphi \| a - b \|^2 }{  2 ( \psi \| a - b \| + 2 \bar{u} ) } \bigg)^n.
    %\end{align}
    %This is equivalent to
    %\begin{align}
    %    \| \chi \|_{L^2}^2  
    %    &\geq \frac{K_1 \varphi^n}{2^n}       
    %     \frac{ \| a - b \|^{2n+4} }{   ( \psi \| a - b \| + 2 \bar{u} )^n } .
    %\end{align}
    %Dividing by~$\frac{K_1 \varphi^n}{2^n}$ and 
    Taking the~$n^{th}$ root yields
    %\begin{align}
    %    \frac{\| \f{\cdot}{\tz} - \h{\cdot}{\tz} \|_{L^2}^2 2^n}{K_1 \varphi^n}
    %    &\geq        
    %     \frac{ \| a - b \|^{2n+4} }{   ( \psi \| a - b \| + 2 \bar{u} )^n } .
    %\end{align}
    %Taking the~$n^{th}$ root of both sides
    %\begin{align}
    %    \sqrt[n]{\frac{\| \f{\cdot}{\tz} - \h{\cdot}{\tz} \|_{L^2}^2 2^n}{K_1 \varphi^n}}
    %    &\geq        
    %     \sqrt[n]{\frac{ \| a - b \|^{2n+4} }{   ( \psi \| a - b \| + 2 \bar{u} )^n }} .
    %\end{align}
    %This is equivalent to
    %\begin{equation}
         %\frac{\sqrt[n]{\| \f{\cdot}{\tz} - \h{\cdot}{\tz} \|_{L^2}^2 2^n}}{\sqrt[n]{K_1 \varphi^n}}
        %&\geq        
         %\frac{ \sqrt[n]{\| a - b \|^{2n+4}} }{ \sqrt[n]{  ( \psi \| a - b \| + 2 \bar{u} )^n }}, \\
    %     \frac{ 2 \sqrt[n]{\| \f{\cdot}{\tz} - \h{\cdot}{\tz} \|_{L^2}^2 }  }{ \varphi \sqrt[n]{K_1}}
    %    \geq        
    %     \frac{ \| a - b \|^{2 + \frac{4}{n}} }{  \psi \| a - b \| + 2 \bar{u} }.
    %\end{equation}
    %Rearranging the equation we reach
    \begin{equation}
    %     \frac{ 2 \psi \sqrt[n]{\| \f{\cdot}{\tz} - \h{\cdot}{\tz} \|_{L^2}^2 }  }{ \varphi \sqrt[n]{K_1}}  \| a - b \|  \\
    %     +  \frac{ 4 \bar{u} \sqrt[n]{\| \f{\cdot}{\tz} - \h{\cdot}{\tz} \|_{L^2}^2 }  }{ \varphi \sqrt[n]{K_1}} 
    %    \geq  \| a - b \|^{2 + \frac{4}{n}} \\
     \| a - b \|^{2 + \frac{4}{n}} - \frac{ 2 \psi \sqrt[n]{\| \chi \|_{L^2}^2 }  }{ \varphi \sqrt[n]{K_1}}  \| a - b \| 
     - \frac{ 4 \bar{u} \sqrt[n]{\| \chi \|_{L^2}^2 }  }{ \varphi \sqrt[n]{K_1}} \leq 0. \label{eq:1021}
    \end{equation}
    A sufficient condition for~\eqref{eq:1021} is 
    %\begin{align}
    %\begin{equation}
         $\| a - b \|^{2 + \frac{4}{n}} - \frac{ 4 \bar{u} \sqrt[n]{\| \chi \|_{L^2}^2 }  }{ \varphi \sqrt[n]{K_1}} 
         \leq 0$.
    %\end{equation}
    %\end{align}
    Solving for~$\| a - b \|$ gives the result. 
    %\begin{multline}
         %\| a - b \|^{2 + \frac{4}{n}}   \leq \frac{ 4 \bar{u} \sqrt[n]{\| \f{\cdot}{\tz} - \h{\cdot}{\tz} \|_{L^2}^2 }  }{ \varphi \sqrt[n]{K_1}} \\
         %\| a - b \| \leq \left( \frac{ 4 \bar{u} \sqrt[n]{\| \f{\cdot}{\tz} - \h{\cdot}{\tz} \|_{L^2}^2 }  }{ \varphi \sqrt[n]{K_1}} \right)^{\frac{n}{2n+4}} \\
        %\| a - b \| \leq \left( \frac{ 4 \bar{u}   }{ \varphi } \right)^{\frac{n}{2n+4}} \left( \frac{ \| \f{\cdot}{\tz} - \h{\cdot}{\tz} \|_{L^2}^2  }{  K_1 } \right)^{\frac{1}{2n+4}}.
    %\end{multline}
    %Replacing~$a = \argmin_{x \in \X} \f{x}{\tz}$ and $b = \argmin_{x \in \X} \h{x}{\tz}$ yields the result.
    \hfill $\blacksquare$
% \end{appendice} 





































    


==> Lemmas/15-relatingProblems.tex <==
\subsection{Proof of Theorem~\ref{thm:2}} \label{lem:relate}








































% \end{appendice}
